Adaptive Discretization for Model-Based Reinforcement Learning

We introduce the technique of adaptive discretization to design an efficient model-based episodic reinforcement learning algorithm in large (potentially continuous) state-action spaces. Our algorithm is based on optimistic one-step value iteration extended to maintain an adaptive discretization of the space. From a theoretical perspective we provide worst-case regret bounds for our algorithm which are competitive compared to the state-of-the-art model-based algorithms. Moreover, our bounds are obtained via a modular proof technique which can potentially extend to incorporate additional structure on the problem. From an implementation standpoint, our algorithm has much lower storage and computational requirements due to maintaining a more efficient partition of the state and action spaces. We illustrate this via experiments on several canonical control problems, which shows that our algorithm empirically performs significantly better than fixed discretization in terms of both faster convergence and lower memory usage. Interestingly, we observe empirically that while fixed-discretization model-based algorithms vastly outperform their model-free counterparts, the two achieve comparable performance with adaptive discretization.

==> parts/partitionexample.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,310); %set diagram left start at 0, and has height of 310

%Shape: Square [id:dp8353167847374121] 
\draw   (50,20) -- (290,20) -- (290,260) -- (50,260) -- cycle ;
%Straight Lines [id:da9444912394077154] 
\draw    (170,20) -- (170,260) ;
%Straight Lines [id:da13817653510361905] 
\draw    (50,140) -- (290,140) ;
%Straight Lines [id:da5928470356620699] 
\draw    (230,20) -- (230,140) ;
%Straight Lines [id:da1153443192808774] 
\draw    (170,80) -- (290,80) ;
%Shape: Circle [id:dp2861072568795213] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.4 ] (490,60) .. controls (490,48.95) and (498.95,40) .. (510,40) .. controls (521.05,40) and (530,48.95) .. (530,60) .. controls (530,71.05) and (521.05,80) .. (510,80) .. controls (498.95,80) and (490,71.05) .. (490,60) -- cycle ;
%Shape: Circle [id:dp2776483980932096] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.4 ] (460,130) .. controls (460,118.95) and (468.95,110) .. (480,110) .. controls (491.05,110) and (500,118.95) .. (500,130) .. controls (500,141.05) and (491.05,150) .. (480,150) .. controls (468.95,150) and (460,141.05) .. (460,130) -- cycle ;
%Shape: Circle [id:dp8327130019060791] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.4 ] (520,130) .. controls (520,118.95) and (528.95,110) .. (540,110) .. controls (551.05,110) and (560,118.95) .. (560,130) .. controls (560,141.05) and (551.05,150) .. (540,150) .. controls (528.95,150) and (520,141.05) .. (520,130) -- cycle ;
%Shape: Circle [id:dp3571591451672438] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.4 ] (580,130) .. controls (580,118.95) and (588.95,110) .. (600,110) .. controls (611.05,110) and (620,118.95) .. (620,130) .. controls (620,141.05) and (611.05,150) .. (600,150) .. controls (588.95,150) and (580,141.05) .. (580,130) -- cycle ;
%Shape: Circle [id:dp7738675368603907] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.4 ] (400,130) .. controls (400,118.95) and (408.95,110) .. (420,110) .. controls (431.05,110) and (440,118.95) .. (440,130) .. controls (440,141.05) and (431.05,150) .. (420,150) .. controls (408.95,150) and (400,141.05) .. (400,130) -- cycle ;
%Shape: Circle [id:dp8126032897461677] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.4 ] (430,200) .. controls (430,188.95) and (438.95,180) .. (450,180) .. controls (461.05,180) and (470,188.95) .. (470,200) .. controls (470,211.05) and (461.05,220) .. (450,220) .. controls (438.95,220) and (430,211.05) .. (430,200) -- cycle ;
%Shape: Circle [id:dp29453391058515477] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.4 ] (490,200) .. controls (490,188.95) and (498.95,180) .. (510,180) .. controls (521.05,180) and (530,188.95) .. (530,200) .. controls (530,211.05) and (521.05,220) .. (510,220) .. controls (498.95,220) and (490,211.05) .. (490,200) -- cycle ;
%Shape: Circle [id:dp34400531809775536] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.4 ] (550,200) .. controls (550,188.95) and (558.95,180) .. (570,180) .. controls (581.05,180) and (590,188.95) .. (590,200) .. controls (590,211.05) and (581.05,220) .. (570,220) .. controls (558.95,220) and (550,211.05) .. (550,200) -- cycle ;
%Shape: Circle [id:dp1768229297347641] 
\draw  [fill={rgb, 255:red, 126; green, 211; blue, 33 }  ,fill opacity=0.4 ] (370,200) .. controls (370,188.95) and (378.95,180) .. (390,180) .. controls (401.05,180) and (410,188.95) .. (410,200) .. controls (410,211.05) and (401.05,220) .. (390,220) .. controls (378.95,220) and (370,211.05) .. (370,200) -- cycle ;
%Straight Lines [id:da9411563154014155] 
\draw    (490,70) -- (420,110) ;
%Straight Lines [id:da410964094319219] 
\draw    (530,70) -- (600,110) ;
%Straight Lines [id:da09935958292754599] 
\draw    (500,80) -- (480,110) ;
%Straight Lines [id:da22411263968286188] 
\draw    (520,80) -- (540,110) ;
%Straight Lines [id:da5638154619759843] 
\draw    (460,140) -- (390,180) ;
%Straight Lines [id:da6422175974350504] 
\draw    (500,140) -- (570,180) ;
%Straight Lines [id:da10758112021502075] 
\draw    (490,150) -- (510,180) ;
%Straight Lines [id:da4414952018490621] 
\draw    (470,150) -- (450,180) ;
%Straight Lines [id:da9572555574912298] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (190,260) -- (190,20) ;

% Text Node
\draw (191,238.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$X^{k}_{h}$};
% Text Node
\draw (165,272.4) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{S}$};
% Text Node
\draw (21,122.4) node [anchor=north west][inner sep=0.75pt]    {$\mathcal{A}$};
% Text Node
\draw (149,120.4) node [anchor=north west][inner sep=0.75pt]    {$B_{1}$};
% Text Node
\draw (203,60.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$B_{21}$};
% Text Node
\draw (203,120.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$B_{23}$};
% Text Node
\draw (263,60.4) node [anchor=north west][inner sep=0.75pt]    {$B_{22}$};
% Text Node
\draw (263,120.4) node [anchor=north west][inner sep=0.75pt]    {$B_{24}$};
% Text Node
\draw (149,240.4) node [anchor=north west][inner sep=0.75pt]    {$B_{3}$};
% Text Node
\draw (269,240.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$B_{4}$};
% Text Node
\draw (409,121.4) node [anchor=north west][inner sep=0.75pt]    {$B_{1}$};
% Text Node
\draw (529,122.4) node [anchor=north west][inner sep=0.75pt]    {$B_{3}$};
% Text Node
\draw (589,122.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$B_{4}$};
% Text Node
\draw (469,122.4) node [anchor=north west][inner sep=0.75pt]    {$B_{2}$};
% Text Node
\draw (499,52.4) node [anchor=north west][inner sep=0.75pt]    {$B_{0}$};
% Text Node
\draw (377,191.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$B_{21}$};
% Text Node
\draw (437,190.4) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$B_{22}$};
% Text Node
\draw (497,191.4) node [anchor=north west][inner sep=0.75pt]    {$B_{23}$};
% Text Node
\draw (557,191.4) node [anchor=north west][inner sep=0.75pt]    {$B_{24}$};
% Text Node
\draw (51,262.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (276,262.4) node [anchor=north west][inner sep=0.75pt]    {$1$};
% Text Node
\draw (36,242.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (36,22.4) node [anchor=north west][inner sep=0.75pt]    {$1$};


\end{tikzpicture}


==> parts/related_work_short.tex <==
% \subsection{Related Work}
% \label{sec:related_work_short}

\textbf{Related Work}.  There is an extensive literature on model-based reinforcement learning; below, we highlight the work which is closest to ours, but for more extensive references, see~\cite{sutton2018reinforcement} for RL, and~\cite{bubeck2012regret,aleks2019introduction} for bandits (and a longer discussion in \cref{sec:related_work}).

Recently there has been a surge in theoretical analysis of nonparametric algorithms for RL in continuous spaces.  These algorithms all require mild local assumptions on the underlying process, most commonly that the $Q$ function is Lipschitz continuous with respect to a given metric.  For example, some work considers nearest-neighbour methods for deterministic, and infinite horizon discounted settings~\cite{yang2019learning,shah2018q}.  Other work assumes access to a generative model instead of the online setting considered here~\cite{kakade2003exploration,henaff2019explicit}.  The work closest to ours concerns algorithms with provable guarantees for continuous state-action settings (see also~\cref{tab:comparison_of_bounds}).  In model-free settings, tabular algorithms have been adapted to continuous state-action spaces via fixed discretization (i.e., $\epsilon$-nets)~\cite{song2019efficient}. In model-based settings, researchers have tackled continuous spaces via kernel methods, based on either a fixed discretization of the space \cite{lakshmanan2015improved}, or more recently, without resorting to discretization~\cite{domingues2020regret}. While the latter does learn a data-driven representation of the space via kernels, it requires solving a complex optimization problem at each step, and hence is efficient mainly for finite action sets (more discussion on this is in \cref{sec:main_results}).
Finally, adaptive discretization has been successfully implemented in model-free settings~\cite{Sinclair_2019, cao2020provably}, and this provides a good benchmark for our algorithm, and for comparing model-free and model-based algorithms.
